Fairness Evaluation in Presence of Biased Noisy Labels

Risk assessment tools are widely used around the country to inform decision making within the criminal justice system. Recently, considerable attention has been devoted to the question of whether such tools may suffer from racial bias. In this type of assessment, a fundamental issue is that the training and evaluation of the model is based on a variable (arrest) that may represent a noisy version of an unobserved outcome of more central interest (offense). We propose a sensitivity analysis framework for assessing how assumptions on the noise across groups affect the predictive bias properties of the risk assessment model as a predictor of reoffense. Our experimental results on two real world criminal justice data sets demonstrate how even small biases in the observed labels may call into question the conclusions of an analysis based on the noisy outcome.

==> experiments.tex <==
 \textbf{(A) Error rates.} {\it If the reoffense rate was equal across races, would disparities disappear?} \\
The impossibility results of \citet{kleinberg2016inherent,chouldechova2017fairlong} tell us that not all parities can be satisfied when base rates differ across groups.  Naturally, one might expect disparities to disappear if rates were equalized. Figure \ref{fig:metric-disp-plot} shows the possible values of $PPV(\alpha_0, \alpha_1)$, $FPR(\alpha_0, \alpha_1)$  and $FNR(\alpha_0, \alpha_1)$ for the COMPAS data having fixed $\alpha = 0.12$ to equalize the ``true'' recidivism rates.\footnote{Technically we are overloading $\alpha$ here to now refer to the sample proportion \mbox{$\#\{Y^*_i = 0, Y_i = 1\} / n_w$}.} We see that for most values of $\alpha$ disparities are even \textit{larger} than what is observed.  We see that while there exist values of $\alpha_1$ under which the ``true'' metric for white defendants would equal the observed (and assumed ``true'') metric for black defendants, the equalizing value of $\alpha_1$ differs across the metrics. Why do disparities persist? 
They persist because of the irreducible disparity in the proportion of defendants in each group that are classified as high risk, that is $\E[\hat{Y}|A=b]- \E[\hat{Y}|A=w]\neq 0$; as observed in \citet{berk2017fairness}, an instrument for which this is not satisfied generally cannot simultaneously achieve parity across metrics. 

{\it What level of $\alpha$ is needed to achieve parity on at least one metric?}\\
Figure \ref{fig:bounds_error_rates} shows the theoretical bounds (yellow lines) provided by Theorem \ref{prop:fpr_fnr_ppv_bounds} as functions of $\alpha$ for the white population, and the metrics for the black population (grey lines) on the COMPAS data. We emphasize the regions highlighted in red, which indicate areas where the true disparity in metrics could be of a different sign than what is observed.  This plot also shows that parity on the true $FPR$ is infeasible in this data at the given choice of classification threshold. 


\begin{figure}
\centering
  \begin{subfigure}[t]{0.48\textwidth}
  \centering
    \includegraphics[width=5cm, height=4cm]{metric_disp_alpha_markup.pdf}
    \caption{$M$ (orange lines) and $M^*$ (grey lines) for white, and $M^*$ (solid dots) for black population in the COMPAS data. $M$ and $M^*$ are true and observed values of $PPV,\; FPR,\; FNR$; $\alpha=0.12$.}
 \label{fig:metric-disp-plot}
  \end{subfigure}\hfill
  \centering
  \begin{subfigure}[t]{0.48\textwidth}
  \centering
   \includegraphics[width=4cm, height=4cm]{figures/Bounds_error_rates.pdf}
\caption{Lower ($M^L$) and upper ($M^U$) bounds for $FPR_w,\; FNR_w,\; PPV_w$ in COMPAS data as described by Theorem \ref{prop:fpr_fnr_ppv_bounds}. Red areas correspond to regions where $\text{sign}(M_w-M_b)\neq \text{sign}(M_w^*-M^*_b)$.}
\label{fig:bounds_error_rates}
  \end{subfigure}
  \caption{Reanalysis of predictive parity and error rate balance for the COMPAS instrument.}
\end{figure}

\textbf{(B) AUC.} The observed $AUC$ for both the black and white defendant population is around $0.69$. Evaluating the bounds from the proposition, we find that for $\alpha=0.05$ and $\alpha=0.12$, the true $AUC_w$ is bounded between $[0.63, 0.76]$ and $[0.51, 0.84]$ respectively. These bounds are very wide, but they can be narrowed if assumptions on the noise are made.


\textbf{(C) Calibration} {\it What is the smallest $\alpha$ necessary to either break or achieve calibration?} \\
\textbf{(C.1) Logistic regression on COMPAS data.} Figure \ref{fig:bounds_coefficient} shows the achievable regions for the coefficients of $A$ in the COMPAS data for $0 \le \alpha\le 0.16$. The green and red areas correspond to regions where the race coefficient is and is not statistically significant, respectively.  Recall that non-significance of the race coefficient indicates that the model is well-calibrated. In this analysis, we find that a TVB level as low as $\alpha = 0.07$ might be sufficient for COMPAS to \textit{fail} the calibration test across all possible noise processes of that magnitude.  At a noise level of only $\alpha=0.04$, calibration might also fail for certain noise processes of this magnitude. Note that our analytic results present bounds not just on the race coefficient but also on the score coefficient in the model. We present the two-dimensional bounds in Section \ref{sec:extra_exp_logistic} of the Supplement. 
%Although the region identified by the analytical bounds for the coefficients of $S$ and $A$ is wide, experimentally we show that, for fixed $\alpha$, the two coefficients appear to be linearly related. % the experiment is reported in the appendix
% Furthermore, assuming less extreme hidden recidivism mechanisms, we find that the coefficient of $S$ is generally not as sensitive to TVB as the bounds might suggest. For instance, if we select hidden recidivists uniformly at random from the white population where $Y^* = 0$, that is if we assume label-dependent noise, we find that the coefficient of $S$ remains close to what is observed.  This is not surprising, since the random flipping mechanism should have little effect on the coefficient of $S$ (compared to flipping the highest or lowest scoring cases) while still having a large effect on the coefficient of $A$. In the Appendix 

\textbf{(C.2) Chi-squared test on Sentencing Commission data.} 
% Figure \ref{fig:chisq_shifts} (left) shows the observed recidivism rates for black and white defendants across the range of the COMPAS decile score. When we apply the chi-squared test to test for calibration, we find that the COMPAS instrument appears well-calibrated with respect to race $(T = 9.36, p-value = 0.49)$. However, applying our method to \textit{maximize} the test statistic, we find that the presence of just $N_h = 20$ hidden recidivists is sufficient to break calibration. This is achieved when all hidden recidivists are located in score level 8. Looking at the data, this is unsurprising. Score level $8$ already has the largest observed discrepancy with the black defendant recidivism rate. Pushing this discrepancy further will rapidly cause the test to reject. \ref{fig:chisq_shifts} (right) shows the minimal shift necessary to break calibration when we impose a \textit{proportionality constraint} that prohibits allocations that concentrate too much on a single bin. Specifically, we require that $h_k \le \epsilon n^{(k)}_{w1}$.  This ensures that the proportion of true recidivists that are hidden \textit{in any score bin} is no greater than $\epsilon$.  For our experiment we take $\epsilon = 0.1$.  Under this constraint, we find that $N_h = 30$ are sufficient to break calibration, obtaining $T = 19.4$, $p$-value $=0.035$. These are allocated as $h = (0,  0,  0,  0,  0,  12,  9,  9,  0,  0)$.
%
The right panel of Figure \ref{fig:chisq_shifts} shows the observed recidivism rates for black and white defendants across the range of the decile score we constructed based on the sentencing commission (SC) data.  Unlike in the COMPAS example, we find that the SC score shows clear evidence of poor calibration $(T = 164, p-value \approx 0)$.  The RAI underestimates risk of rearrest for white offenders relative to black offenders across the range of score levels.  This effect is especially pronounced in the highest scores.  Applying our method to \textit{minimize} the test statistic, we find that just $N_h = 1001$ hidden recidivists are sufficient to achieve calibration.  While this may seem like a large number, there are $n_w = 31607$ white offenders in the data, of which $n_{w1} = 13552$ are observed to reoffend.  Thus the minimizing allocation requires only that $1001 / (13552 + 1001) = 6.9\%$ of all true recidivists go unobserved.  The minimizing allocation, represented in the left panel of Figure~\ref{fig:chisq_shifts}, is $h = (41,  35,  46,   0,   0, 224, 186, 197, 170, 102)$.

%\textbf{Noise rates.} Here we estimate noise rates as in Proposition \ref{prop:estimation_noise}, for black and white population. We split into train and test sets, fit and tune with cross-validation race-specific classifiers, and repeat the training/estimation procedure on 20 random train/test splits. The following estimates (standard deviation) correspond to white and black populations parameters: 0.13 (0.11) and 0.07 (0.06) with extreme gradient boosted trees, 0.18 (0.08) and 0.08 (0.05) with logistic regression, 0.12 (0.10) and 0.12 (0.08) with knn.

%\textbf{Simulation.} {\it Is label noise the only source of bias in the data?} Clearly, no. Label noise induces bias in As a simple example, consider two defendants $b,w$ that, ceteris paribus, have $x_b=x_w>0$ (true prior number of crimes), but $x^*_b>x^*_w\geq 0$ (observed). Trivially, if $p^*$ is increasing in $x$, then $b$ will suffer from {\it compounding injustice} \citetp{hellman2017indirect} compared to $w$; equivalently unjustified disparate impact arises. We simulate \fixme{Discuss simulation and add figure to previous page.}% add simulation (also using COMPAS data?)
% idea assume some form for label noise and see how it impact
%%%% OR 
% otherwise talk about inclusion or not of rate when you're not correcting for label noise: which one is better? Something from my own notes + think about simulation




\begin{figure}
\centering
  \begin{subfigure}[t]{0.38\textwidth}
   \includegraphics[width=\linewidth]{figures/calibration_logistic_bound_race.pdf}
\caption{Bounds for the race coefficient as in Proposition~\ref{prop:logistic_bound}. The red (green) region corresponds to coefficients whose $p$-value is (\textit{not}) statistically significant.}
  \label{fig:bounds_coefficient}
  \end{subfigure} \hspace{2em}
  \begin{subfigure}[t]{.48\linewidth}
  \centering
\includegraphics[width=0.48\linewidth]{calib_pcs_original.pdf}
\includegraphics[width=0.48\linewidth]{calib_pcs_uncon.pdf}
  \caption{Calibration comparison for original data (left) and minimal shifts (right) to achieve calibration between black (grey) and white (orange) population in the Sentencing Commission data.}
  \label{fig:chisq_shifts}
\end{subfigure}
\caption{Reanalysis of calibration properties of (a) COMPAS and (b) a risk assessment instrument constructed using the sentencing commission's data.  In (a), the red region corresponds to settings where the target variable bias is sufficient to reverse the conclusion that the COMPAS tool is well-calibrated with respect to race.}
\end{figure}




==> extra_experiments.tex <==
%%%%%%%%%%%%%%%%
% DATA description
For one of the analyses in Section \ref{sec:chisq} we rely on a private data set provided by a state level sentencing commission.  That dataset contains information on all offenders sentenced in the state's criminal courts between 2001-2004.  The data allows us to observe rearrest outcomes for all offenders during the first three years upon release from incarceration.  We construct a recidivism risk score by modeling the 3-year recidivism outcome using regularized logistic regression as a function of offender age, sex, and several dozen criminal history variables.  To facilitate comparison with the COMPAS score, we convert the predicted probabilities to a decile score.  Our empirical results are based on applying this score to a held out set of $55031$ offenders, of whom 65.4\% are white and the remainder are black.  

% Might naively expect that all parities would hold if we had observed reoffense instead of rearrest.





%%%%%%%%%%%%%%%%%%% AUC




%%%%%%%%%%%%%%%%%%%%%%%% calibration testing with logisitic regression
\begin{figure}[t]
\includegraphics[width=\linewidth]{bounds_coefficients.pdf}
\caption{Outer red curves show the bounds guaranteed by Proposition~\ref{prop:logistic_bound} for different choices of $\alpha$ (which are labeled on the curves). Blue rectangles correspond to analytical bounds, though empirically we can verify that the coefficients must in fact lie on the dashed diagonals.  Orange curve shows coefficients under a ``random'' mechanism where we assume each observation with $Y^* = 0$ was equally likely to be a hidden recidivist.  Points marked with an X correspond to values of $\alpha_w$  where the $p$-value of $\beta_A$ is \textit{not} statistically significant.  These are values of $\alpha_w$ where we would conclude that $S$ is well calibrated with respect to $A$ as a predictor of the true $Y$.   }
\label{fig:bounds_coefficients}
\end{figure}

% \begin{figure}[t]
% \includegraphics[width=\linewidth]{pvalue_simple_model.pdf}
% \caption{P-value of race coefficient \noterf{(LRT and z-statistic are the same here, right, up to one of them being signed?)} $\alpha$.}
% \label{fig:bounds_pvalue}
% \end{figure}


Figure \ref{fig:bounds_coefficients} shows the achievable regions for the coefficients of $S$ and $A$ in the COMPAS data for $0 \le \alpha_w \le 0.16$.  The plot also indicates with X's points where the true coefficient $\beta_A$ would not be statistically significant.  These correspond to settings where we would conclude that COMPAS is well calibrated with respect to $A$ (race) as a predictor of $Y$ (reoffense).  In this analysis, we find that a TVB level as low as $\alpha_w = 0.08$ would be sufficient for COMPAS to \textit{fail} the calibration test across all hidden recidivism mechanisms. 

Although the region identified by the analytical bounds is wide, experimental results show that the coefficients are considerably further constrained.  First, we find empirically that no matter the indexes of the hidden recidivists, the coefficients at a given $\alpha_w$ always lie on the diagonal connecting the lowest and highest bounds that we find.   Furthermore, assuming less extreme hidden recidivism mechanisms, we find that the coefficient of $S$ is generally not as sensitive to TVB as the bounds might suggest. For instance, if we select hidden recidivists uniformly at random from the white population where $Y^* = 0$, we find that the coefficient of $S$ remains close to what is observed (this is the orange line).  This is not surprising, since the random flipping mechanism should have little effect on the coefficient of $S$ (compared to flipping the highest or lowest scoring cases) while still having a large effect on the coefficient of $A$.  


The analysis in this section provides us with insight into how TVB affects the simplest logistic regression based test of calibration.  An issue with this test is that the logistic model is likely to be misspecified, thus resulting in a test that fails to detect certain types of deviation from calibration.  In the next section we consider a more robust calibration test that has power against deviations that might go undetected by the logistic regression test.  




%%%%%%%%%%%%%%%% experiments for calibration with chi-squared test

\subsubsection{Experiments on the Sentencing Commission data} Figure \ref{fig:chisq_shifts}(c) shows the observed recidivism rates for black and white defendants across the range of the decile score we constructed based on the sentencing commission  (SC) data.  Unlike in the COMPAS example, we find that the SC score shows clear evidence of poor calibration $(T = 164, p-value \approx 0)$.  The RAI underestimates risk of rearrest for white offenders relative to black offenders across the range of score levels.  This effect is especially pronounced in the highest scores.  Applying our method to \textit{minimize} the test statistic, we find that just $N_h = 1001$ hidden recidivists are sufficient to achieve calibration.  While this may seem like a large number, there are $n_w = 31607$ white offenders in the data, of which $n_{w1} = 13552$ are observed to reoffend.  Thus the minimizing allocation requires only that $1001 / (13552 + 1001) = 6.9\%$ of all true recidivists go unobserved.  The minimizing allocation, represented in Figure\ref{fig:chisq_shifts}(d), is $h = (41,  35,  46,   0,   0, 224, 186, 197, 170, 102)$.


% \begin{verbatim}
% You will want to use your own wording, but:
% For the original data you gave me, you have:
% T = 9.364765 on 10 DF
% p = 0.4978709

% If you allow 20 moves, you have:
% T = 27.85458
% p = 0.00190458
% achieved by moving 20 people at score level 8
% \end{verbatim}

%\begin{table}[ht]
%\centering 
%\begin{table}[ht]
%\begin{tabular}{|l|cc|}
%\hline
%$S = k$ & $Y^* = 0$ &  $Y^* = 1$ \\ \hline
%$A = w$ & $n^{(k)}_{w0}$ & $n^{(k)}_{w1}$ \\ 
%$A = b$ & $n^{(k)}_{b0}$ & $n^{(k)}_{b1}$ \\
%\hline
%\end{tabular}
%\caption{Contingency table for observations in score level $S \in \{1, \ldots, |S| \}$ for testing  $H_0: Y^* \perp A \mid S$ with the chi-squared test.  \textcolor{red}{Note to Max: }We've been using $Y^*$ for the observed outcome and $Y$ for the true, though this is getting annoying and I'm thinking of switching it. Feel free to use whichever notation you want.  Just let me know what you do.  }
%\label{tab:chisq_obs}
% \end{table}


% In terms of Table \ref{tab:chisq_true}, the chi-squared statistic based on the observed $Y^*$ can be written as
% \begin{align*}
%   T = \sum_{k} &\left(
%   \frac{\left(\nk_{w1} +h_k - 
%   \left(\nk_{w1}+\nk_{b1}+h_k\right)\left(\nk_{w0}+\nk_{w1}\right)/\nk\right)^2}{\left(\nk_{w1}+\nk_{b1}+h_k\right)\left(\nk_{w0}+\nk_{w1}\right)/\nk}\right.\\
%   &+ \frac{\left(\nk_{b1}  - 
%   \left(\nk_{w1}+\nk_{b1}+h_k\right)\left(\nk_{b0}+\nk_{b1}\right)/\nk\right)^2}{\left(\nk_{w1}+\nk_{b1}+h_k\right)\left(\nk_{b0}+\nk_{b1}\right)/\nk}\\
%   &+ \frac{\left(\nk_{w0} -h_k - 
%   \left(\nk_{w0}+\nk_{b0}-h_k\right)\left(\nk_{w0}+\nk_{w1}\right)/\nk\right)^2}{\left(\nk_{w0}+\nk_{b0}-h_k\right)\left(\nk_{w0}+\nk_{w1}\right)/\nk}\\
%   &\left.+\frac{\left(\nk_{b0} - 
%   \left(\nk_{w0}+\nk_{b0}-h_k\right)\left(\nk_{b0}+\nk_{b1}\right)/\nk\right)^2}{\left(\nk_{w0}+\nk_{b0}-h_k\right)\left(\nk_{b0}+\nk_{b1}\right)/\nk}
%   \right)
% \end{align*}
% where $\nk = \nk_{w0}+\nk_{w1}+\nk_{b0}+\nk_{b1} = \#\{i : S_i = k\}$ is the total number of defendants in score bin $k$.  

% \bigskip
% Alternative writings
% \begin{align*}
%   T = \sum_{k}\sum_{r\in\{w,b\}} &\left(
%   \frac{\left(\nk_{r1} +h_k \Ind_{r=w}- 
%   \left(\nk_{w1}+\nk_{b1}+h_k\right)\left(\nk_{r0}+\nk_{r1}\right)/\nk\right)^2}{\left(\nk_{w1}+\nk_{b1}+h_k\right)\left(\nk_{r0}+\nk_{r1}\right)/\nk}\right.\\
%   &+ \left.\frac{\left(\nk_{r0} -h_k\Ind_{r=w} - 
%   \left(\nk_{w0}+\nk_{b0}-h_k\right)\left(\nk_{r0}+\nk_{r1}\right)/\nk\right)^2}{\left(\nk_{w0}+\nk_{b0}-h_k\right)\left(\nk_{r0}+\nk_{r1}\right)/\nk}\right)
% \end{align*}

% \bigskip
% or another
% \begin{align}
% \label{eq:chisq_statistic}
%   T = \sum_{k}\sum_{\stackrel{r\in\{b,w\}}{y\in\{0,1\}}} 
%   \frac{\left(\nk_{ry} +h_k\Ind_{r=w} - 
%   \left(\nk_{wy}+\nk_{by}+ s_y h_k\right)\left(\nk_{r0}+\nk_{r1}\right)/\nk\right)^2}{\left(\nk_{wy}+\nk_{by}+ s_yh_k\right)\left(\nk_{r0}+\nk_{r1}\right)/\nk}
% \end{align}
% where $s_y = \begin{cases} 1 & y=1 \\ -1 & y=0\end{cases}$.









%%%%%%%%%%%%%%%%%%%%%%%%% model training who are the likely hidden recidivists?

It is clear that under feature-dependent noise such an ``extreme'' setting might occur. For instance, suppose that $X \in \{0,1\}$ is a single binary covariate, $p(1) = 1, p(0) = p_0 < 0.5$, and $\gamma(1) = 0.4, \gamma(0) = 0$.  This gives $p^*(1) = 0.5$ and $p^*(0) = p_0 < 0.5 <  0.6 = p^*(1)$.  If we set the classification threshold at $s_{HR} = 0.5$, we would classify everyone with $X = 1$ as high-risk and everyone with $X = 0$ as low-risk.  By construction, we have $\gamma(0) = 0$, meaning that all recidivists with $X = 0$ are observed, whereas some fraction of recidivists with $X = 1$ are hidden.  This in turn means that all hidden recidivists are classified as high-risk ($\alpha_0 = 0$).  A similar construction can be used to produce a case where $\alpha_1 = 0$, which corresponds to all hidden recidivists being classified as low-risk. Such an example is admittedly highly contrived and unlikely to reflect any real world scenario, but it can not by ruled out. Indeed, the noise in uniquely bounded by
\[
p^*(x)=(1-\gamma(x))p(x)\leq 1-\gamma(x)\implies \gamma(x)\leq 1-p^*(x).
\]








 To model a more plausible scenario, we consider a setup in which we have a single feature $X \sim Unif[0,1]$, $p(x) = x$, and two forms for the likelihood of getting caught function: $\gamma^{Inc,b}(x) = 1-(b+1)x/(1 + bx)$, and \\ \mbox{$\gamma^{Dec, b}(x) = 1-(b+1)(1-x)/(1 + b(1-x))$}.  The ``Increasing'' setting $\gamma^{Inc,b}$ is one where the likelihood of getting caught increases with the likelihood of reoffense $p(x)$, with the functional form of the relationship governed by the parameter $b$.  The ``Decreasing'' setting has the likelihood of getting caught decreasing with the likelihood of reoffense.  We equalize the proportion of of high-risk and low-risk cases by thresholding $p^*(x)$ at its median value in each simulation.  Figure \ref{fig:prophr_plot} shows a plot of how the fraction of hidden recidivists that get classified as high-risk varies with $b$.  Values $>0.5$ on this plot can be interpreted as settings where $\alpha_1 > \alpha_0$; a value of $1$, though never achieved, would correspond to the case $\alpha_0 = 0$.  This suggests that, in general, the hidden recidivists are likely to be scattered across the range of the score $S$, and are thus unlikely to concentrate entirely in the extremes of $S$.  In other words, the worst-case bounds presented in Section \ref{sec:sensitivity} are, unsurprisingly, likely to be overly conservative.  






%\begin{figure}[t]
%\includegraphics[width=\linewidth]{hidden_recid_prop.pdf}
%\caption{Proportion of hidden recidivists classified as high risk under %different choices of $\gamma_{11}$.  }
%\label{fig:prophr_plot}
%\end{figure}


% Despite the unobservable nature of the censoring process, one might hope to restrict the choice for some form of the distribution of $S|Y=1,Y^{*}=0$ with high confidence. We now show that, without any further knowledge on $Y$, nothing can be inferred.\\
% % treating s as a deterministic mechanism of X
% The score $s(X)$\footnote{In full generality, s is a function of both X and A.} can be decomposed as
% \begin{gather}\label{eq:decomposition_score}
% s(X)=\gamma(X)\pi(X)
% \end{gather}
% where $\gamma(X)=\E[Y^{*}|Y=1,X]$ and $\pi(X)=\E[Y|X]$. The expression \ref{eq:decomposition_score} allows us to identify the region of interest
% \begin{gather}
% R_{t}=\{X\in\mathbb{X}:E[Y|Y^{*}=0,X]>t\}
% \end{gather}
% for some $t\in[0,1]$. If $t=0$, the condition entails the identification of all $X$ for which the average hidden recidivism is non zero; in this case,
% \begin{gather}
% \Pb(s(X)>t|X\in R_{0})=\frac{\E_{X}[\pi(X)(1-\gamma(X))\mathbbm{1}(s(X)>t)]}{\E_{X}[\pi(X)(1-\gamma(X))]}.
% \end{gather}
% which is equivalent to $1-FNR^{h}$. Although the numerator can be upper bounded, the denominator can be arbitrarily large depending on the form of $\gamma$ and $\pi$: for instance, if $\pi$ is assumed to be constant, individuals only differ in the probability of getting caught.\\

% We illustrate two toy examples where a distribution for $\gamma$ is assumed. 1. Let $\gamma(X)\sim \mathcal{U}[s(X),1]$, and consequently the probability density function of $\pi(X)$ has the form $s(X)/[(1-s(X))z^{2}]$ with $z\in[s(X),1]$. 2. Consider $\gamma(X)\sim s(X)+(1-s(X))B$ where $B\sim Beta(2,5)$. Although the assumptions reflect very different beliefs - in the first example we assume the process could be of any magnitude, while in the second we assume that some subjects may never get caught while being repeated offenders- show that, apart from naively avoiding scenarios likely to be paradoxical as in the example 2., the main takeaway is to convey the idea that it is hard to agree on common form for such distributions.\\





%%%%%%%%%%%%%%% model training biased
\subsection{Disparate impact resulting from training with biased data} \label{sec:disp_impact}

One of the main takeaways from our discussion of predictive parity and error rate balance in Section~\ref{sec:fpr_fnr_ppv_bounds} is that disparities will generally continue to persist even if we hypothesize that the true reoffense rates are equal across groups.  This is due to the fact that a greater proportion of black defendants get classified as high risk, and the classifications $\hat Y$ are unaffected when adjusting for TVB in the evaluation.   In other words, this is due to the irreducible disparity in \mbox{$\P(\hat Y = 1\mid A = b) - \P(\hat Y = 1 \mid A = w)$}.  But where does this disparity come from?  In this section we discuss how training a model with biased data leads to (unjustified) disparate impact.  Our main contribution is an empirical analysis of the worst-case disparate impact that can result from training on data affected by TVB.  

\begin{figure*}[t]
\begin{subfigure}{.5\linewidth}
  \centering
\includegraphics[width=\linewidth]{KS_discrimination_black.pdf}
  \caption{Maximal disparate impact against black defendants.}
  \label{fig:disc_black}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
\includegraphics[width=\linewidth]{KS_discrimination_white.pdf}
  \caption{Maximal disparate impact against white defendants.}
  \label{fig:disc_white}
\end{subfigure}
\caption{Densities for the signed maximal disparate impact measures (SDMI) for the experiment described in Section~\ref{sec:disp_impact}. The model for $S$ is a logistic regression on age, priors count, count of juvenile felonies, sex, and race; the threshold $t_0$ is chosen to satisfy $p_{01}=p_{10}$ for $\alpha_w=0$.}
\label{fig:signed_KS}
\end{figure*}

We begin by introducing our measure of worst-case disparate impact.  Given an RAI, $S$, we can look at the distribution of $S$ across the group $A = b$ an $A = w$.  Let $F_{S_b}$ and $F_{S_w}$ be the cdfs of the score in each group.  For $t_0 \in [0,1]$, we define the \textit{signed maximal disparate impact} (SMDI) measures as,
\begin{align}
D^+_{S_b,S_w}&=\sup_{t\geq t_{0}}F_{S_b}(t)-F_{S_w}(t),  \\
D^-_{S_b,S_w}&=\sup_{t\geq t_{0}}F_{S_w}(t)-F_{S_b}(t).
\end{align}
In the case $t_0 = 0$, these are equivalent to signed versions of the familiar Kolmogorov-Smirnov statistic. The SMDI measures quantify the maximal level of disparate impact that can be achieved by a decision-maker applying a threshold $s_{HR} \ge t_0$ to $S(X,A)$ in classifying defendants as high-risk. Positive values of $D^-$ indicate disparate impact against black defendants, while positive values of $D^+$ indicate disparate impact against white defendants.    Our experiments study how the SMDI is affected as we retrain an RAI on the COMPAS data while synthetically decreasing the disparity in recidivism rate between the black and white defendants.  

% where $F_{p}$ is the cumulative distribution function of $p$. If $p_{1}$ and $p_{2}$ are respectively $p(X,a)$ and $p(X,b)$, the signed KS statistic quantifies the maximal discrimination that can be achieved by a malevolent decision-maker. In case of $p_{1}=p(X,A)$ and $p_{2}=p^{*}(X,A)$, its value indicates the worst-case scenario for the disparate impact between true and observed outcome. In other terms, we are interested in the minimization of the maximal unfairness, defined as statistical parity, that can be achieved.\\

\textit{Experimental setup.}  In this COMPAS data experiment we randomly select a subset of $\ceil{n\alpha}$ white defendants for whom we observe $Y^* = 0$ and flip their outcome in the data to $Y = 1$.  This process mimics `uncovering' hidden recidivists.  We then fit a logistic regression model to the resulting data to obtain a score $S(X,A)$.  From there we calculate the SMDI measures.  This process is repeated $1000$ times for each $\alpha$ on a grid from $0.01$ to $0.12$.  Recall that $\alpha = 0.12$ equalizes recidivism rates across the two racial groups.  

\emph{Experimental results and discussion.} Figure~\ref{fig:signed_KS} summarizes the results.  This Figure shows densities of the SDMI statistics across the range of $\alpha$ values considered.  We see from \ref{fig:signed_KS}(a) that as we get closer to equalizing recidivism rates through the random flipping mechanism, the maximal disparate impact against black defendants decreases substantially.  Indeed, \ref{fig:signed_KS}(b) shows that for the largest values of $\alpha$ considered, we observe many realizations where there is a possibility of disparate impact against white defendants.  The main takeaway is that training a model on data affected by TVB can produce much larger levels of disparate impact than what could be expected if the model were trained on the true outcome $Y$.  

TVB is one of many reasons for why an RAI might result in disparate impact.  Not all disparate impact is unjustified or indicative of bias or discrimination.  As noted in \citet{Corbett-Davies:2017:ADM:3097983.3098095,corbett2018measure} we would not expect the maximal disparity to be $0$ even if the recidivism rate were equal across groups and the training data were observed without bias.  This is because any difference in the distribution of $S$ across groups could produce some level of disparate impact.  Another possibility is that we could have differential measurement bias in the observed features $X^*$.  This could lead to artificially inflated (or deflated) scores for one of the groups, which in turn would result in large disparate impact.  As noted in \citet{corbett2018measure}, assuming TVB is not an issue, differential measurement bias in $X^*$ can be attenuated by constructing models that explicitly use $A$ as an input.  For instance, one could construct separate models for the two groups.  

% In general, any different distribution of the scores between the groups above the threshold $t_{0}$ possibly generates disparate impact. As an example, consider two groups showing the same recidivism rate: even if we had access to an oracle providing the information $p^{*}(X,a)=p^{*}(X,b)$, not correcting for sample bias in the observed $X^{*}$ might lead to some worst-case disparity between the groups in case the distribution was different\footnote{It would inevitably lead to disparate impact if the bias in $X$ affected $Y|X*$.}; in absence of such a correction, individual classifiers, for each group separately, can be trained to overcome this issue. \\


% In presence of target variable bias, fairness of the classifier with respect to $Y$ is of primary interest. While section \ref{sec:sensitivity} contained a discussion regarding how the fairness properties of the same classifier transfer from $Y^{*}$ to $Y$, we now study if such guarantees hold when the classifier is retrained on $Y$. In this subsection we propose a measure for the assessment of worst-case disparate impact, showing its connection to other typical metrics and an application.\\

% The assumption about some form for the distribution of $Y^{*}|Y$ is complementary to a certain characterization for the distribution of the scores $S(X,A)$. Through a notion of distance, disparate impact can be assessed and typical metrics of fairness can be roughly reconstructed; in the recidivism context, we are interested in some disparity in the high scores. While such a choice of the distribution is arbitrary and dependent on the context, throughout the section we will often refer to a ``random'' mechanism to indicate sampling $(X_1,\dots,X_K)\sim X|Y^{*}=0$ and setting $(Y_{1},\dots,Y_{K})=\boldsymbol{1}$.\\

% The above mentioned measure is an signed Kolmogorov-Smirnov statistic: for some $t_{0}\in[0,1]$, it is defined as
\begin{figure}[t]
\includegraphics[width=\linewidth]{disparate_impact_modeling_choice.pdf}
\caption{Mean signed SMDI metric $D^{-}$ between black and white population for different values of $\alpha_w$ and several classifiers. The models shown are logistic regression and random forest (rf). Feature sets are: (1) age and priors count, (2) only sex; +A indicates that the protected attributed is also included as a feature.}
\label{fig:KS_modeling}
\end{figure}


% The statistic links to the usual metrics: for fixed $t$, it corresponds to statistical parity, and, also conditionally on the positive class, it reflects an equal opportunity criterion. Consequently, if the statistic is close to zero, then fairness based on such metrics will be guaranteed.\\




% Consider the case of $\E[Y^{*}|A=a]\leq E[Y^{*}|A=b]$ and $\alpha_{w}>0$, while $\alpha_{b}=0$. As detailed above, for a classifier trained on $(Y,X,A)$, as $\alpha_{a}$ is increased, the signed KS statistic would likely shrink; however, we show that for a random hidden recidivism mechanism this not always happens to be the case. Figure \ref{fig:signed_KS} shows density estimation for the KS statistics under such mechanisms for varying levels of $\alpha$ based on a logistic regression model.\footnote{Up to $\alpha_{a}=0.07$, for COMPAS data a random mechanism is approximately equivalent to a mechanism equalizing the marginal rates on past criminal history (priors count).} Such randomness together with sample bias in the regressor is the cause of the unresolved discrimination for $\alpha=0.12$, when rates of recidivism are equalized. Although the derivation of non-trivial\footnote{Their form varies case by case. However, typically assuming that all similar subjects, characterized by some $X=x$ such that $S(X)<\epsilon$, are hidden recidivists leads to a larger statistic.} analytical bounds is infeasible, notice that being agnostic about the mechanism still results in narrow confidence intervals for the mean of the statistic. Modeling choices should be guided by the evaluation of the magnitude of disparate impact in presence of target variable bias: while classifiers in our simulations generally show substantial reduction of the statistic, the selection of regressors appears to be the most important factor.\\


The choice of model and features can have a significant effect on the level of disparate impact resulting from an RAI.  While the direct inclusion of protected attributes often faces opposition, we demonstrate next that this strategy can help mitigate disparate impact resulting from data bias.  Figure \ref{fig:KS_modeling} shows the mean value of the signed SDMI statistic $D^-$ for different choices of model $S$ across a range of $\alpha$ values.  This experiment applies the same random flipping mechanism as described earlier in the section.  What we find is that when $A$ is not included in the model, the SMDI against black defendants does not approach $0$ even as the recidivism rates across groups become equalized.    

% that doing so Many authors have often advocated against the inclusion of the protected attribute in the set of regressors; however, we argue that, without any knowledge on the mechanism, such a covariate, or a strong proxy, might help avoid disparate impact.  Intuitively, under a random mechanism, typically $\E[p(x,a)]\neq p(x,b)$\footnote{The expectation is taken with respect to the mechanism.}: therefore a classifier would likely account for the such difference between the groups only by modeling the protected attribute. The  bad behavior of the classifier is directly attributable to modeling misspecification, as the omission of $A$, based on the observed data where it might not be informative, is inadequate. On the other hand, if a mechanism satisfying $p^{*}(x,a)\leq \E[p(x,a)]\leq p(x,b)$ is considered, then the inclusion of race would likely not be needed. 

% In figure \ref{fig:KS_modeling} we show the signed KS statistic evaluated on different classifier for COMPAS data: the exclusion of race in the model penalizes the disparity between the groups, regardless of the level of unobserved recidivism assumed. More importantly, bias in the regressor does not allow for low values of the statistic, unless some correction is made; in particular, notice the logistic regression model on sex and race: as they are only affected by covariate shifting, the difference in distributions between the groups does allow for a gradual decrease of the statistic. However, for $\alpha$ large enough, mean disparate impact drops dramatically.\\




% notice that logistic regression (2)+A at a certain value of alpha


% The main takeaway is that bias in the regressor is a necessary condition for target variable bias: while certain covariates uniquely suffer of covariate shifting (e.g. sex), bias in others also affects the conditional (e.g. prior criminal history). In the latter case, even if $p(y|X,a)=p(y|X,b)$, conditioning on $X^{*}$ will inevitably lead to some magnitude of disparate impact. Although one may tailor ad-hoc corrections of the distribution, any effort may still be nullified by model misspecification.\\
 













%\note{This section should present results of what happens when we train on biased vs unbiased data.  Things that can go in here:}

%\begin{itemize}
%	\item FPR, FNR, PPV in the setting where we account for retraining (considering $p$, $p^*$ and $\gamma$.  
%	\item Analyses of $p$ vs $p^*$ and how this might help refine our bounds from the sensitivity analysis section
%    \item Modified KS statistic and connections to disparate impact
%\end{itemize}

%Despite any careful attempt to avoid unfairness in policy decisions, hidden recidivism might endanger the efforts: even accounting for a correction of the outcome, the classical properties of classifier often do not persist if the regressor is biased. The first part of this section is devoted to a short overview of such issue; the second subsection contains our proposal of a criterion for the assessment of fairness in presence of sample bias.\\

%\subsection{Bias in the regressor}
%Sample bias in the recidivism context represents an inextricable problem: given the impossibility of recovering the distribution of $(X,Y)$, no correction can be designed; luckily, such pessimism is not always warranted.\\

%We are interested in two cases of bias in the regressor:
%\begin{enumerate}
%\item $P_{X}\neq P_{X^{*}}$ and $P_{Y|X=x}=P_{Y|X^{*}=x}$, also known as covariate shift;
%\item $P_{X}\neq P_{X^{*}}$ and $P_{Y|X=x}=P_{Y|X^{*}=x}$.
%\end{enumerate}




%%%%%%%%%%%%%%%%%%%%%%%%%%% on the estimation of the noise rate




%%%%%%%%%%%%%%%% estimation of noise rates

\textbf{Estimation of noise rates.} 
Implement EM for the a logitic noise and plot it in the figure.\\
We also estimate noise rates as in Proposition \ref{prop:estimation_noise}, for black and white population. We split the data into train and test sets, fit and tune with cross-validation race-specific classifiers, and repeat the training/estimation procedure on 20 random train/test splits. The following estimates (standard deviation) correspond to white and black populations parameters: 0.13 (0.11) and 0.07 (0.06) with extreme gradient boosted trees, 0.18 (0.08) and 0.08 (0.05) with logistic regression, 0.12 (0.10) and 0.12 (0.08) with knn.

==> training.tex <==
One of the main takeaways from our discussion of predictive parity and error rate balance in Section~\ref{sec:evaluation} is that disparities will generally continue to persist even if we hypothesize that the true reoffense rates are equal across groups.  This is due to the fact that in the sensitivity analysis approach the classification $\hat{Y}$ is unaffected by TVB, and the proportion of individuals classified as high risk is larger in the black population.  In other words, this is due to the irreducible disparity in \mbox{$\E[\hat Y \mid A = b] - \E[\hat Y \mid A = w]$}.  But where does this disparity come from?  In this section we discuss how differential measurement in $X^*$ is inevitably tied to TVB, leading to unjustified disparate impact.  Our main contribution is an empirical analysis of the worst-case disparate impact that can result from training on data affected by TVB.

We begin by introducing our measure of worst-case disparate impact.  Given a RAI represented by $S$, we can look at its distribution conditional on the race group $A$.  Let $F_{S_b}$ and $F_{S_w}$ be the cdf's of the score in each group.  For $t_0 \in [0,1]$, we define the \textit{signed maximal disparate impact} (SMDI) measures as
\begin{gather}
D^+_{S_b,S_w}\coloneqq \sup_{t\geq t_{0}}F_{S_b}(t)-F_{S_w}(t),  \\
D^-_{S_b,S_w}\coloneqq \sup_{t\geq t_{0}}F_{S_w}(t)-F_{S_b}(t).
\end{gather}
In the case of $t_0 = 0$, the SMDI measures are equivalent to signed versions of the familiar Kolmogorov-Smirnov statistic. These measures quantify the maximal level of disparate impact that can be achieved by a decision-maker applying a threshold $s_{HR} \ge t_0$ to $S(X,A)$ in classifying defendants as high-risk. Positive values of $D^+$ indicate disparate impact against white defendants, while positive values of $D^-$ indicate disparate impact against black defendants.

% where $F_{p}$ is the cumulative distribution function of $p$. If $p_{1}$ and $p_{2}$ are respectively $p(X,a)$ and $p(X,b)$, the signed KS statistic quantifies the maximal discrimination that can be achieved by a malevolent decision-maker. In case of $p_{1}=p(X,A)$ and $p_{2}=p^{*}(X,A)$, its value indicates the worst-case scenario for the disparate impact between true and observed outcome. In other terms, we are interested in the minimization of the maximal unfairness, defined as statistical parity, that can be achieved.\\

Our experiments study how the SMDI is affected as we retrain a RAI on the COMPAS data while synthetically decreasing the disparity in recidivism rates between the black and white defendants. We randomly select a subset of $\ceil{n\alpha}$ white defendants for whom we observe $Y^* = 0$ from the data and set their outcome to $Y = 1$. This process mimics `uncovering' hidden recidivists.\footnote{If the noise rate $\gamma$ is thought to be constant within the white population, then our method has a close connection to the method of label-dependent costs of \citep{natarajan2013learning} described in the Supplement.} % note: we need to make sure that we do not assume constant noise, otherwise one might just argue that we could have trained an unbiased weighted logistic regression: sampling the hidden recidivists means that we could also be taking into account other configurations of the noise
We then fit a logistic regression model to the resulting data to obtain a score $S(X,A)$, and compute the SMDI measures. This process is repeated $1000$ times for each $\alpha$ on a grid from $0.01$ to $0.12$.  Recall that $\alpha = 0.12$ equalizes recidivism rates across the two racial groups.

\begin{figure*}[t]
\centering
\begin{subfigure}{.5\linewidth}
  \centering
\includegraphics[width=\linewidth]{KS_discrimination_black.pdf}
  \caption{Maximal disparate impact against black defendants.}
  \label{fig:disc_black}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
\includegraphics[width=\linewidth]{KS_discrimination_white.pdf}
  \caption{Maximal disparate impact against white defendants.}
  \label{fig:disc_white}
\end{subfigure}
\caption{Density estimates for the signed maximal disparate impact measures (SDMI) for the experiment described in Section~\ref{sec:training}. The model for $S$ is a logistic regression on age, priors count, count of juvenile felonies, sex, and race; the threshold $t_0$ is chosen to satisfy $p_{01}=p_{10}$ for $\alpha^w=0$.}
\label{fig:signed_KS}
\end{figure*}


{\it Would disparate impact be reduced if the model were trained on the true outcome $Y$?}\\
Figure~\ref{fig:signed_KS} summarizes the results of the experiment.  This Figure shows densities of the SDMI statistics across the range of $\alpha$ values considered.  On the one hand, we see from \ref{fig:signed_KS}(a) that as we get closer to equalizing recidivism rates through the random sampling mechanism, the maximal disparate impact against black defendants decreases substantially.  However, it never reaches zero. On the other hand, \ref{fig:signed_KS}(b) shows that for the largest values of $\alpha$ considered, we observe many realizations where there is possibility of disparate impact against white defendants. 

There are two main takeaways from this experiment. First, the resulting level of maximal disparate impact for a model trained on data affected by TVB will  typically be larger than for a model trained on clean data. This conclusion seems natural since we are equalizing recidivism rates. Second, disparate impact could possibly be observed at any level of $\alpha$. This fact should be surprising as we would expect that, training on clean data, disparate should be driven to zero for some choice of $\alpha$. Why doesn't this occur? TVB is only one of many reasons why a RAI might result in disparate impact.  Not all disparate impact is unjustified or indicative of bias or discrimination.  As noted in \citet{Corbett-Davies:2017:ADM:3097983.3098095,corbett2018measure} we would not expect the maximal disparity to be $0$ even if the recidivism rates were equal across groups and the training data were observed without bias.  This is because any difference in the distribution of $S$ across groups could produce some level of disparate impact.  Another possibility is that we could have differential measurement bias in the observed features $X^*$.  This could lead to artificially inflated (or deflated) scores for one of the groups, which in turn would result in large disparate impact. In presence of differential measurement bias in $X^*$, the choice of model and features can have a significant effect on the level of disparate impact resulting from an RAI, as our next experiment shows.


\begin{figure}[t]
\centering
\begin{subfigure}{.5\linewidth}
  \centering
\includegraphics[width=\linewidth]{disparate_impact_modeling_choice_minus.pdf}
  \caption{Mean SMDI metric $D^{-}$ as a function of $\alpha$.}
  \label{fig:disc_black}
\end{subfigure}%
\begin{subfigure}{.5\linewidth}
  \centering
\includegraphics[width=\linewidth]{disparate_impact_modeling_choice_plus.pdf}
  \caption{Mean SMDI metric $D^{+}$ as a function of $\alpha$.}
  \label{fig:disc_white}
\end{subfigure}
\caption{Mean signed SMDI metric $D^{-}$ (a) and $D^{+}$ (b) between black and white population for different values of $\alpha^w$ and several classifiers. The models shown are logistic regression (logistic) and random forest (rf). The feature sets are: (1) age and priors count, (2) only sex; +A indicates that the protected attributed is also included as a feature.}
\label{fig:KS_modeling}
\end{figure}
%%% fix this figure



Figure \ref{fig:KS_modeling} shows the mean value of the signed SMDI statistics $D^-$ and $D^+$ for different choices of model $S$ across a range of $\alpha$ values.  This experiment applies the same random sampling mechanism described earlier in the section; the sampling is repeated 50 times for every combination of model, feature set, and $\alpha$. The feature sets (1), age and priors count, and (2), only sex, have been selected such that (2) represents a simpler model, and only in (1) the conditional distributions $Y|X$ and $Y|X^*$ are likely to differ.\footnote{In the machine learning literature, the bias in $(Y,X^*)$, where $X^*$ belongs to the feature set (2), is typically referred to as {\it covariate shift}.} The models considered are logistic regression (logistic) and random forest (rf). Figure \ref{fig:KS_modeling} (b) reveals that the mean SMDI statistic $D^{+}$, that is the maximal disparate impact against white defendants, is positive only for a few values of $\alpha$; however, $D^{+}$ (b) appears to be always smaller than $D^-$ (a). There are three important facts to notice in Figure \ref{fig:KS_modeling} (a). First, for the set of features (1), the mean maximal level of disparate impact against black defendants decreases with $\alpha$ only if $A$ is included in the model. Indeed, as also noted in \citet{corbett2018measure}, if TVB is not an issue, differential measurement bias in $X^*$ can be attenuated by constructing models that explicitly use $A$ as an input, or by fitting separate models for the groups. Second, if $A$ is included, then models using feature set (2) show higher values of the SMDI metric compared to the models using (1). This fact might be a consequence either of model complexity or, as we hypothesize, difference in the type of bias in $(Y,X^*)$. Third, for the same feature set, the magnitude of the SMDI metric for logistic regression and random forest appears to greatly differ. 
The main takeaway from this experiment is that, although the direct inclusion of protected attributes often faces opposition, it can help mitigate disparate impact resulting from data bias.




% notice that logistic regression (2)+A at a certain value of alpha


% The main takeaway is that bias in the regressor is a necessary condition for target variable bias: while certain covariates uniquely suffer of covariate shifting (e.g. sex), bias in others also affects the conditional (e.g. prior criminal history). In the latter case, even if $p(y|X,a)=p(y|X,b)$, conditioning on $X^{*}$ will inevitably lead to some magnitude of disparate impact. Although one may tailor ad-hoc corrections of the distribution, any effort may still be nullified by model misspecification.\\
 













%\note{This section should present results of what happens when we train on biased vs unbiased data.  Things that can go in here:}

%\begin{itemize}
%	\item FPR, FNR, PPV in the setting where we account for retraining (considering $p$, $p^*$ and $\gamma$.  
%	\item Analyses of $p$ vs $p^*$ and how this might help refine our bounds from the sensitivity analysis section
%    \item Modified KS statistic and connections to disparate impact
%\end{itemize}

%Despite any careful attempt to avoid unfairness in policy decisions, hidden recidivism might endanger the efforts: even accounting for a correction of the outcome, the classical properties of classifier often do not persist if the regressor is biased. The first part of this section is devoted to a short overview of such issue; the second subsection contains our proposal of a criterion for the assessment of fairness in presence of sample bias.\\

%\subsection{Bias in the regressor}
%Sample bias in the recidivism context represents an inextricable problem: given the impossibility of recovering the distribution of $(X,Y)$, no correction can be designed; luckily, such pessimism is not always warranted.\\

%We are interested in two cases of bias in the regressor:
%\begin{enumerate}
%\item $P_{X}\neq P_{X^{*}}$ and $P_{Y|X=x}=P_{Y|X^{*}=x}$, also known as covariate shift;
%\item $P_{X}\neq P_{X^{*}}$ and $P_{Y|X=x}=P_{Y|X^{*}=x}$.
%\end{enumerate}
